Controlled Language Generation for Language Learning Items

This work aims to employ natural language generation (NLG) to rapidly generate items for English language learning applications: this requires both language models capable of generating fluent, high-quality English, and to control the output of the generation to match the requirements of the relevant items. We experiment with deep pretrained models for this task, developing novel methods for controlling items for factors relevant in language learning: diverse sentences for different proficiency levels and argument structure to test grammar. Human evaluation demonstrates high grammatically scores for all models (3.4 and above out of 4), and higher length (24%) and complexity (9%) over the baseline for the advanced proficiency model. Our results show that we can achieve strong performance while adding additional control to ensure diverse, tailored content for individual users.

==> sections/tasks.tex <==
\section{Tasks}
    At its base form, our task is to generate a sentence using a list of concepts: the resulting sentence should contain relevant vocabulary from the concept list, but is otherwise unconstrained. Consider the following examples:
    
    \begin{itemize}
        \item concept concept concept $\rightarrow$ sentence
        \item concept concept concept $\rightarrow$ sentence
        \item concept concept concept $\rightarrow$ sentence
    \end{itemize}

    \subsection{Difficulty-controlled generation}
    
    Another option is to control for the difficulty or complexity of the output. By difficulty we are  here referring the ability level required to understand the generated sentence: in this subtask, we aim to provide the model with additional information that will influence the generation to be aimed at learners with a particular ability level. This allows us to be better tailor the generated outputs to specific users and/or applications. 
    
    For our difficulty levels, we use CEFR (*), a system for evaluating the complexity of documents. These labels are, in increasing order of difficulty, A1, A2, B1, B2, C1, and C2. Our goal is to be able to start with a list of concepts and generate a sentence at the appropriate difficulty level.


    \subsection{Argument structure control}
    As a secondary task, would also like to be able to constrain the argument structure of the generated sentences. To do this, we aim to be able to determine for any given concept in the input what semantic role that concept should be play in the output text. This gives two key advantages: we can ensure the semantic viability of generations in which the concepts make more sense in particular roles, and we can extend the variety of sentences generated by varying the semantic roles of the arguments. Consider the following generation:
    
    \begin{itemize}
        \item $\textrm{\{dog, chase, cat\}} \rightarrow {\textrm{(a) the dog chased the cat} \atop \textrm{(b) the cat chased the dog}}$ 
    \end{itemize}
    
    As the concepts are unordered, the model can generate both sentences where (a) the dog is chasing the cat and where (b) the cat is chasing the dog. Stereotypically, we would expect (a), but (b) is a viable reading. By enforcing the semantic roles of the concepts, either with the dog or the cat as the agent, our aim is to be able to more concretely choose which output we'd like to see.
    

\Debanjanin{Here too we need to find some citations from the language learning + skill space. }

